Measures in Visualization Space

Measurement is an integral part of modern science, providing the fundamental means for evaluation, comparison, and prediction. In the context of visualization, several different types of measures have been proposed, ranging from approaches that evaluate particular aspects of individual visualization techniques, their perceptual characteristics, and even economic factors. Furthermore, there are approaches that attempt to provide means for measuring general properties of the visualization process as a whole. Measures can be quantitative or qualitative, and one of the primary goals is to provide objective means for reasoning about visualizations and their effectiveness. As such, they play a central role in the development of scientific theories for visualization. In this chapter, we provide an overview of the current state of the art, survey and classify different types of visualization measures, characterize their strengths and drawbacks, and provide an outline of open challenges for future research.

==> preamble.tex <==
%
\newcommand{\strCompare}[1]{%
  \ifthenelse{\equal{\detokenize{#1}}{\detokenize{Glossary}}}
    {TRUE}
    {FALSE}%
}
%
\makeatletter
\g@addto@macro{\maketitle}{\def\author#1{\def\@author{#1}}}
\newcommand*{\extendsectlevel}[1]{%
  \expandafter\newcommand\expandafter*\csname saved@#1\endcsname{}%
  \expandafter\let\csname saved@#1\expandafter\endcsname\csname #1\endcsname
  \expandafter\renewcommand\expandafter*\csname #1\endcsname{%
    \expandafter\let\csname author@#1\endcsname\@author
    \@ifstar
      {\csname star@#1\endcsname}%
      {\@dblarg{\csname opt@#1\endcsname}}%
  }%
  \expandafter\newcommand\expandafter*\csname star@#1\endcsname[1]{%
    \csname saved@#1\endcsname*{##1%
      \expandafter\ifx\csname author@#1\endcsname\@empty\else
        \hfill\linebreak{\normalsize
          \textmd{\textit{\csname author@#1\endcsname}}}%
      \fi
    }%
  }%
  \expandafter\newcommand\expandafter*\csname opt@#1\endcsname[2][]{%
    \csname saved@#1\endcsname[{##1%
      \expandafter\ifx\csname author@#1\endcsname\@empty\else
%        \enskip\textmd{\textit{(\csname author@#1\endcsname)}}%
% >>> UN/COMMENT the above line to enable/disable author names in the TOC
      \fi
    }]{##2%
      \expandafter\ifx\csname author@#1\endcsname\@empty\else
        \hfill\linebreak{\normalsize
          \textmd{\textit{\csname author@#1\endcsname}}}%
      \fi
    }%
  }%
}
\extendsectlevel{chapter}
\extendsectlevel{section}
%\extendsectlevel{subsection}
\makeatother
%
\addtolength{\marginparwidth}{10mm}
%
\makeatletter
\def\contact{\xdef\@thefnmark{}\@footnotetext}
\makeatother
%
\usepackage{etoolbox}
\newbool{createReferencesFromBBL}
\booltrue{createReferencesFromBBL}
%
\newcounter{chaptersave}
%
\newbool{createChapterReferences}
\boolfalse{createChapterReferences}
%\booltrue{createChapterReferences}

\renewcommand\thesection{\arabic{chapter}.\arabic{section}}

% Custom blank footnote
\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}
